PIM Is All You Need: A CXL-Enabled GPU-Free System for Large Language Model Inference

Large Language Model (LLM) inference uses an autoregressive manner to generate one token at a time, which exhibits notably lower operational intensity compared to earlier Machine Learning (ML) models such as encoder-only transformers and Convolutional Neural Networks. At the same time, LLMs possess large parameter sizes and use key-value caches to store context information. Modern LLMs support context windows with up to 1 million tokens to generate versatile text, audio, and video content. A large key-value cache unique to each prompt requires a large memory capacity, limiting the inference batch size. Both low operational intensity and limited batch size necessitate a high memory bandwidth. However, contemporary hardware systems for ML model deployment, such as GPUs and TPUs, are primarily optimized for compute throughput. This mismatch challenges the efficient deployment of advanced LLMs and makes users pay for expensive compute resources that are poorly utilized for the memory-bound LLM inference tasks. We propose CENT, a CXL-ENabled GPU-Free sysTem for LLM inference, which harnesses CXL memory expansion capabilities to accommodate substantial LLM sizes, and utilizes near-bank processing units to deliver high memory bandwidth, eliminating the need for expensive GPUs. CENT exploits a scalable CXL network to support peer-to-peer and collective communication primitives across CXL devices. We implement various parallelism strategies to distribute LLMs across these devices. Compared to GPU baselines with maximum supported batch sizes and similar average power, CENT achieves 2.3$\times$ higher throughput and consumes 2.9$\times$ less energy. CENT enhances the Total Cost of Ownership (TCO), generating 5.2$\times$ more tokens per dollar than GPUs.

==> 2-motivation-backup.tex <==
\section{Motivation}

The key motivation driving our work is the \textbf{large memory capacity} requirements and the \textbf{low GPU compute utilization} in LLM inference. The increased demand for memory capacity limits inference batch sizes, leading to low compute utilization. Further, low compute utilization is caused by the low operational intensity of decoder-only LLMs and insufficient memory bandwidth in existing GPU systems.

% LLMs are large
LLM parameter size has witnessed an exponential increase from Billion to Trillion magnitudes, far surpassing previous machine learning (ML) models. In addition, the context windows that modern LLMs support range from 128K to 1M~\cite{gpt4-turbo, gemini-pro}, enabling the ability to understand and generate longer contents.
% , as shown in Table~\ref{tab:context_wiindow}. 
The long context window results in a large KV cache. Further, the KV cache is unique for each user, which requires large memory capacity when scaling up the inference batch size. 

% \begin{table}[htbp]
%     \vspace{-4mm}
%     \centering
%     \caption{Modern LLM Context Window Size}
%     \vspace{-2mm}
%     \scriptsize
%     \label{tab:context_wiindow}    
%     % \setlength{\tabcolsep}{2.5pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{1.1}
%     \scalebox{1.15} {
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%         \multirow{3}{*}{Model} & \multirow{3}{*}{\shortstack{Meta \\ Llama 2}} & \multirow{3}{*}{\shortstack{Google \\ Gemini \\ 1.0 Pro}} & \multirow{3}{*}{\shortstack{OpenAI \\ GPT-4 \\ Turbo}} & \multirow{3}{*}{\shortstack{Anthropic \\ Claude 3}} & \multirow{3}{*}{\shortstack{Google \\ Gemini \\ 1.5 Pro}}  \\
%          & & & & & \\
%          & & & & & \\
%         \hline
%         \hline
%         \multirow{2}{*}{\shortstack{Context \\ Window}} & \multirow{2}{*}{\shortstack{4K \\ ~\cite{touvron2023llama}}} & \multirow{2}{*}{\shortstack{32K \\ ~\cite{gemini-models}}} & \multirow{2}{*}{\shortstack{128K \\ ~\cite{gpt4-turbo}}} & \multirow{2}{*}{\shortstack{200K \\ ~\cite{claude}}} & \multirow{2}{*}{\shortstack{1M \\ ~\cite{gemini-pro}}} \\
%          & & & & & \\
%         \hline
%     \end{tabular}
%     }
    
%     \vspace{-2mm}
% \end{table}

Figure~\ref{fig:Context_Length} studies the memory capacity requirements, and its adverse impact on batch size using vLLM~\cite{vLLM}, the \sota{} inference serving framework for GPUs. vLLM 
% employs the PagedAttention algorithm to 
dynamically swaps memory blocks between the host CPU and GPUs, enabling flexible batch sizes that can exceed the physical memory capacity of the GPUs. 
% We study the open-source Llama2-70B model and its. While Llama2-70B only supports 4K context length, its fine-tuned versions support up to 32K~\cite{longlora}. 

% {\fontsize{8pt}{11pt}\selectfont 8pt font size test Memory Requirement}
% \todo{Remove batch size = 1 to increase the font in the figure?}

\begin{figure}[htbp]
% \vspace{-3mm}
\centering
    % \includegraphics[width=8.5cm]{Figure/Context_Length.pdf}
    \includegraphics[width=\columnwidth]{Figure/Context_Length.pdf}
    % \vspace{-3mm}
    \caption{Llama2-70B~\cite{touvron2023llama, longlora} on 4 A100 80GB GPUs}
    \label{fig:Context_Length}
    % \vspace{-3mm}
\end{figure}

In Figure~\ref{fig:Context_Length}, the memory requirements (right y-axis, blue bars) increase with larger batch sizes (x-axis). The inference throughput (left y-axis, dot line) improves with larger batch sizes but reaches a plateau once the memory requirement exceeds the GPU memory size. With the context length increasing, the inference throughput saturates with even smaller batch sizes, from batch=128 at 4K context length to batch=8 at 32K context length. Moreover, LLM inference query latency increases with larger batch sizes, as depicted in Figure~\ref{fig:GPU_utilization}(a). Thus realistic query latency service level agreements (SLA) constraints~\cite{mlperf-sla} further prohibit the use of large batch sizes, especially for longer context lengths.


\begin{figure}[t]
% \vspace{-3mm}
\centering
    % \includegraphics[width=8.5cm]{Figure/GPU_utilization.pdf}
    \includegraphics[width=\columnwidth]{Figure/GPU_utilization.pdf}
    % \vspace{-3mm}
    \caption{(a) Llama2-70B inference query latency increases with larger batches on 4 A100 80GB GPUs,  Prompt size=512, Decoding size=3584. (b) GPU compute utilization is measured by Nvidia Nsight Compute profiler on 4 GPUs for Llama2-70B and 1 GPU for the other two models.}
    \label{fig:GPU_utilization}
    % \vspace{-6mm}
\end{figure}


To accommodate the large memory capacity requirements of LLM inference tasks, multiple GPUs are connected together, which leaves the individual GPU underutilized and significantly drives up the hardware cost. Figure~\ref{fig:GPU_utilization}(b) depicts the GPU compute utilization of three ML models. 
% The decoder-only LLMs' operational intensity remains lower compared to earlier ML models such as BERT~\cite{devlin2018bert} and ResNet~\cite{he2016deep}. 
Encoder-only transformer models such as BERT~\cite{devlin2018bert} process input tokens within a prompt concurrently, forming an input matrix to multiply with the weight matrix (GEMM).
Convolutional Neural Networks (CNNs) such as ResNet~\cite{he2016deep} implement parameter reuse in convolution operations, further increasing their operational intensity.

In decoder-only LLMs, prompt processing (prefill stage) is similar to the encoding process in BERT, however, output tokens are generated sequentially during the decoding stage.
This process results in an input vector that multiplies with the weight matrix (GEMV).
The operational intensity of GEMV is substantially lower than GEMM, underutilizing the massive compute throughput of GPUs.
Furthermore, the operational intensity in LLMs does not scale linearly with batch size because the attention calculations rely on KV caches, which is unique to each batch.
Although 128 batch size and group query attention coalesce GEMVs into GEMM, Llama2-70B only utilizes \textcolor{myblue}{21\% of the GPU's compute throughput.}
% still exhibits half GPU utilization when compared to BERT.
\textcolor{myblue}{Due to the significant lower operational intensity, decoding an output token takes $3.4\times$ longer than encoding a prompt token in the prefill stage.
Hence, this work focuses on the decoding stage of the decoder-only LLMs.}


% Note that the operational intensity of Llama2-70B does not scale linearly with batch size because the attention calculations rely on KV caches. The KV caches are unique to each batch, which prevents GEMVs coalescing into GEMM with batching. 

\todo{Do we need this paragraph? It looks redundant:}
Modern GPUs are equipped with substantial computational resources, offering a high peak compute throughput with a comparably limited memory bandwidth. This makes them over-provisioned for LLM inference with relatively lower operational intensity, leading to low GPU utilization.

% \subsection{PIM Provides High Internal Bandwidth}

% Many PIM architectures place processing units (PU) adjacent to memory banks, enhancing internal bandwidth between the bank and PU. %This surpasses the external bandwidth capabilities of conventional DRAM. 
\textbf{PIM Provides Higher Internal Memory Bandwidth}. 
% PIM has been manufactured in various industrial prototypes.
Table~\ref{tab:hardware_comparison} compares various manufactured industrial PIM prototypes and GPU. 
% with Bfloat16/FP16 compute throughput. 
The internal bandwidth provided by PIM significantly exceeds that of high bandwidth memories (HBM) used in high-end GPUs. For example, GDDR6-based AiM~\cite{aim1, aim2} achieves $16~TB/s$ internal memory bandwidth compared to $2~TB/s$ A100 GPU with five HBM2E memory stacks. This large internal bandwidth coupled with lower operational intensity makes PIM architectures more suitable than GPUs to perform LLM inference tasks. 

%Table~\ref{tab:hardware_comparison} shows that the A100 GPU provides a theoretical maximum operational intensity of $156~Ops/byte$,
%Llama2-70B model has an operational intensity of $1~Op/byte$ in a single batch and $59~Op/byte$ with batch=128, contrasting with BERT and ResNet-152, with operational intensity of $282$ and $346~Ops/byte$, respectively. 

\begin{table}[t]
% \small
\footnotesize
    \centering
    \caption{Hardware System Comparison}
    \label{tab:hardware_comparison}    
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Type & \multicolumn{3}{|c|}{PIM} & GPU   \\
        \hline
        % Name & UPMEM~\cite{upmem} & AiM~\cite{aim1} & FIMDRAM~\cite{fimdram} & A100 \\
        Name & UPMEM & AiM & FIMDRAM & A100 \\
        
        % \multirow{2}{*}{Name} & UPMEM & AiM & FIMDRAM & \multirow{2}{*}{A100} \\
        % & ~\cite{upmem} & ~\cite{aim1} & ~\cite{fimdram} & \\
        \hline
        Mem. Units & 8 channels & 32 ch. & 5 stacks & 5 st. \\
        \hline
        Ex. BW (TB/s) & 0.15 & 1 & 1.5 & 2 \\
        \hline
        In. BW (TB/s) & 1 & 16 & 12.3 & - \\
        \hline
        Capacity (GB) & 64 & 16 & 30 & 80 \\
        \hline
        TFLOPS & 0.5 TOPS~\footnotemark & 16 & 6.2 & 312 \\
        \hline
        Ops/Byte & 0.5 & 1 & 0.5 & 156 \\
        \hline
    \end{tabular}
\end{table}

% \begin{table}[t]
% \footnotesize
%     % \vspace{-4mm}
%     \centering
%     \caption{Hardware System Comparison}
%     % \vspace{-1mm}
%     \label{tab:hardware_comparison}    
%     \setlength{\tabcolsep}{2.8pt} % Default value: 6pt
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{|c|c|c|c|c|c|c|c|}
%         \hline
%         \multirow{3}{*}{Type} & \multirow{3}{*}{Name} & \multirow{3}{*}{\shortstack{Mem. \\ Units}} & \multirow{3}{*}{\shortstack{Ext. \\ BW \\ (TB/s)}} & \multirow{3}{*}{\shortstack{Int. \\ BW \\ (TB/s)}} & \multirow{3}{*}{\shortstack{Memory \\ Capacity \\ (GB)}} & \multirow{3}{*}{\shortstack{Compute \\ Throughput \\ (TFLOPS)}} & \multirow{3}{*}{\shortstack{Operational \\ Intensity \\ (Ops/Byte)}} \\
%          & & & & & & & \\
%          & & & & & & & \\
        
%         \hline 
%         \hline 
%         % \ignore{
%         % & DDR4 & 8 ch & 0.15 & - & 512 & - & - \\
%         % \cline{2-8}
%         % DRAM & GDDR6~\cite{micron-gddr6} & 32 ch & 1 & - & 64 & - & - \\
%         % \cline{2-8}
%         % & HBM2E & 5 st & 2  & - & 80 & - & - \\
%         % \hline
%         % }
%         & UPMEM~\cite{upmem} & 8 ch & 0.15 & 1  & 64 & 0.5 TOPS\footnotemark 
%         & 0.5  \\
%         \cline{2-8}
%         PIM & AiM~\cite{aim1} & 32 ch & 1  & 16 & 16 & 16 & 1  \\
%         \cline{2-8}
%         & FIMDRAM~\cite{fimdram} & 5 st & 1.5 & 12.3 & 30 & 6.2  & 0.5  \\
%         \hline
%         GPU &  A100 & 5 st & 2 & - & 80 & 312  & 156 \\
%         \hline
%         % CPU &  Xeon Max & 8 ch & 0.31 & - & 512  & $\approx$ 10  & 32.5  \\
%         % \hline
%     \end{tabular}
    
%     \vspace{-5mm}
% \end{table}
% \vspace{-7mm}
\footnotetext{UPMEM supports only integer precision, so unit is TOPs.}


%Despite the low operational intensity, the aggregate operations needed for LLM inference are still large. Hence modern CPUs with limited acceleration features and memory bandwidth fall short of the compute resources.



% While PIM's large internal bandwidth aligns well with the requirements of inference tasks, PIM designs typically exhibit low operational intensity. AiM achieves an operational intensity of $1~Ops/Byte$ as only low-intensity compute logic can be fabricated with DRAM processes. Fortunately, these compute resources match the decoder-only LLM requirements.

% \subsection{Hierarchical PIM-PNM architures}
\todo{Avoid selecting thoughts}
UPMEM~\cite{upmem} and FIMDRAM~\cite{fimdram} supports general-purpose operations near memory banks. AiM~\cite{aim1, aim2} applies a domain specific design into near-bank PUs, providing higher compute throughput. Although a custom PU design achieves better performance, it cannot support the entire transformer block without resorting to expensive GPUs.
To balance this trade-off between generality and customization, we propose a \textbf{hierarchical PIM-PNM architecture.} In PIM channels, the near-bank PUs are composed of MAC units, which can efficiently support the GEMV operations in the transformer block. The PNM units are placed near memory channels, comprising accelerators and RISC-V cores to perform infrequent special operations. RISC-V cores provides flexibility and support a diverse range of LLMs. 

% \subsection{CXL Features an Efficient and Scalable Network}

Additionally, an inherent trade-off with PIM is the increased area due to processing units and enabling internal memory access features. This consequently leads to a reduction in memory capacity when compared to equivalent DRAM technologies. For instance, 
DDR4-based UPMEM R-DIMM~\cite{upmem} has 4$\times$ lower memory capacity compared to conventional DDR4 R-DIMMs. 
%\reetu - Upmem uses RDIMM or registered DIMM which comes in smaller sizes than typical unbuffered DIMMs.
GDDR6 channels already have lower memory capacity than DDR4, and GDDR6-based AiM further incurs an area overhead of 25\% due to added computational circuit~\cite{aim2}. 
%4$\times$ compared to highest density GDDR6 chips~\cite{micron-gddr6} available for same I/O pin bandwidth of 16 Gb/s. 
This motivates our proposed architecture that compensates for the reduced memory capacity in PIM by utilizing CXL~\cite{sharma2022compute} based memory expansion. 

\textbf{CXL Features an Efficient and Scalable Network.}
As a low-latency interconnect protocol built on top of the PCIe physical layer, CXL supports peer-to-peer inter-device communication in the 3.0 version~\cite{CXL}. CXL.mem offers an effective solution to connect plenty of memory modules, achieving lower latency than network-based RDMA solutions. The CXL 3.0 protocol can support up to 4,096 nodes, exhibiting better scalability than NVLink. Although NVLink provides higher bandwidth, which is critical in LLM training, CXL network is capable of LLM inference with the mapping strategies introduced in Section~\ref{model mapping}.










% The parameter size of LLMs has witnessed an exponential increase, far surpassing previous machine learning (ML) models.
% However, the decoder-only LLMs' operational intensity remains lower compared to earlier ML models such as BERT~\cite{devlin2018bert} and ResNet~\cite{he2016deep}. In BERT, input tokens within a prompt are processed concurrently, forming an input matrix to multiply with the weight matrix. This parallel processing contrasts with decoder-only LLMs, where tokens are generated one after another in a sequential manner, resulting in an input vector that multiplies with the weight matrix. The operational intensity of vector-matrix multiplication (GEMV) is substantially lower than that of matrix-matrix multiplication (GEMM). Additionally, convolutional neural networks (CNNs), such as ResNet, not only engage in matrix-matrix multiplications but also implement kernel reuse strategies, which further increase the operational intensity. 
% % The comparison above is shown in Figure~\ref{fig:gpu_op_density} (a). 
% With a single batch, Llama2-70B model has an operational intensity of $1~Op/byte$ contrasting with BERT and ResNet-152, with operational intensity of $282$ and $346~Ops/byte$, respectively.


% \begin{figure*}[ht]
% 	\centering
%   	\includegraphics[width=17.5cm]{Figure/Combo_Motivation.pdf}
%   	\vspace{-4mm}
% 	\caption{(a) Llama2-70B uses 4 NVIDIA A100 80GB GPUs while the other two models use a single GPU. Llama2-70B is measured with 128 batches and 4K context length. (b) With larger inference batch sizes (x-axis), memory requirements (right y-axis) increase because KV Caches of each batch are unique. The inference throughput (left y-axis) improves with increasing batch sizes but reaches a plateau once the memory requirement exceeding the GPU memory size. While Llama2-70B only supports 4K context length, its fine-tuned versions support up to 32K context length~\cite{longlora}. With longer context length, the inference throughput saturates with smaller batch sizes. (c) Inference query latency exhibits a linear increase with respect to both batch size and context length.}
% \label{fig:Combo_Motivation}
% \vspace{-6mm}
% \end{figure*}

% Modern GPUs enjoy expansive compute resources, offering a high peak operation throughput at a comparably limited memory bandwidth. Table~\ref{tab:hardware_comparison} shows that A100 GPUs offer $156~Ops/byte$. Thus GPU's compute resources are over-provisioned for LLMs which require a low operational intensity.
% Further, to accommodate large parameter sizes, multiple GPUs are connected together to provide a high aggregate memory capacity, which significantly drives up the cost of inference hardware. In addition, the large KV cache unique to each user requires extra memory capacity (Table~\ref{tab:context_wiindow}), limiting the inference batch size.
% Therefore, we observe that GPUs suffer from significant underutilization for decoder-only LLMs. To illustrate this phenomenon, we measure the GPU utilization using the maximum supported batch size of three models, as shown in Figure~\ref{fig:Combo_Motivation}(a).
% % To illustrate this phenomenon, we measure the utilization of the instruction issue throughput of the NVIDIA A100 GPUs using maximum supported batch size of three machine learning models.
% % Figure~\ref{fig:Combo_Motivation}(a) shows that while BERT and ResNet-152 highly utilize a GPU ($43\%$ and $80\%$), Llama2-70B only utilizes $21\%$ compute throughput of 4 GPUs. 


% Llama2-70B GPU utilization is measured using vLLM~\cite{vLLM}, a state-of-the-art LLM inference serving framework.
% While vLLM uses the PageAttention technique to swap memory blocks between the host CPU and GPUs to support flexible batch sizes, the inference throughput reaches a plateau once the memory requirement exceeds the GPU memory size, as shown in Figure~\ref{fig:Combo_Motivation}(b). 
% % We measure Llama2 70B with 128 batches and 4K context length, where the inference throughput stops increasing.
% Note that with longer context lengths, the inference throughput saturates with smaller batch sizes. 
% % LLMs use key-value caches to store context information.
% The context windows that modern LLMs support are increasing from thousands of tokens to 1 million tokens to understand and generate longer contents, as shown in Table~\ref{tab:context_wiindow}. Figure~\ref{fig:Combo_Motivation}(c) shows that the inference query latency increases with larger batch sizes, detrimentally affecting user experiences. Both longer context length and quality of service (QoS) requirements limit inference batch sizes, making the GPU utilization worse in real world LLM deployments.



% Despite the low operational intensity, the aggregate operations needed for LLM inference are still large. Hence modern CPUs with limited acceleration features and memory bandwidth fall short of the compute resources.

% Many PIM architectures place processing units (PU) adjacent to each memory bank, enhancing internal bandwidth between the bank and PU. %This surpasses the external bandwidth capabilities of conventional DRAM. 
% Table~\ref{tab:hardware_comparison} compares different PIM technologies with their Bfloat16/FP16 compute throughput. The internal bandwidth provided by PIM significantly exceeds that of High Bandwidth Memories (HBM) used in high-end GPUs. For example, GDDR6-based AiM~\cite{aim1, aim2} achieves $32~TB/s$ internal memory bandwidth compared to $2~TB/s$ A100 GPU with five HBM2e memory stacks. While PIM's large internal bandwidth aligns well with the requirements of inference tasks, PIM designs typically exhibit low operational intensity. AiM achieves an operational intensity of $1~Ops/Byte$ as only low-intensity compute logic can be fabricated with DRAM processes. Fortunately, these compute resources match the decoder-only LLM requirements.


% However, an inherent trade-off with PIM is the increased area due to processing units and enabling PIM memory access features. This consequently leads to a reduction in memory capacity when compared to equivalent DRAM technologies. For instance, 
% DDR4-based UPMEM R-DIMM~\cite{upmem} has 4$\times$ lower memory capacity compared to conventional DDR4 R-DIMMs. 
% %\reetu - Upmem uses RDIMM or registered DIMM which comes in smaller sizes than typical unbuffered DIMMs.
% GDDR6 channels already have lower memory capacity than DDR4, and GDDR6-based AiM further incurs an area overhead of 25\% due to added computational circuit~\cite{aim2}. 
% %4$\times$ compared to highest density GDDR6 chips~\cite{micron-gddr6} available for same I/O pin bandwidth of 16 Gb/s. 
% This motivates our proposed architecture that compensates for the reduced memory capacity in PIM by utilizing CXL~\cite{sharma2022compute} based memory expansion. 

% CXL is a low-latency interconnect protocol built on top of the PCIe physical layer, supporting peer-to-peer inter-device communication in the 3.0 version~\cite{CXL}. CXL offers an effective and scalable solution to connect plenty of memory modules, achieving lower latency than network-based RDMA solutions. 
% % Multi-sockets CPUs connected through the UPI protocol also support a large amount of memory modules but use more CPUs as control nodes than CXL-based solutions.

% % [TODO: not cache but inter-device] CXL is a low-latency cache-coherent interconnect built on top of the PCIe physical layer. CXL offers an effective and scalable solution for memory expansion as it supports byte-addressable and CPU cacheable accesses, even though it is built upon PCIe. This allows the host to access any CXL-connected remote memory devices seamlessly and even integrate PCIe storage into a cache-coherent memory space, significantly expanding the available memory~\cite{Jung2022Storage}. 


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

